Developers' Visuo-spatial Mental Model and Program Comprehension

Previous works from research and industry have proposed a spatial representation of code in a canvas, arguing that a navigational code space confers developers the freedom to organise elements according to their understanding. By allowing developers to translate logical relatedness into spatial proximity, this code representation could aid in code navigation and comprehension. However, the association between developers' code comprehension and their visuo-spatial mental model of the code is not yet well understood. This mental model is affected on the one hand by the spatial code representation and on the other by the visuo-spatial working memory of developers. We address this knowledge gap by conducting an online experiment with 20 developers following a between-subject design. The control group used a conventional tab-based code visualization, while the experimental group used a code canvas to complete three code comprehension tasks. Furthermore, we measure the participants' visuo-spatial working memory using a Corsi Block test at the end of the tasks. Our results suggest that, overall, neither the spatial representation of code nor the visuo-spatial working memory of developers has a significant impact on comprehension performance. However, we identified significant differences in the time dedicated to different comprehension activities such as navigation, annotation, and UI interactions.

==> figures/corsi_block.tex <==
\begin{figure}
    \centering
    \includegraphics[scale=0.3]{images/corsi_test.png}
    \caption{Corsi Block Test for Visuospatial working memory.}
    \label{fig:corsi_block_test}
\end{figure}

==> figures/timelines.tex <==
\begin{figure*}
    \centering
    \includegraphics[scale=0.2]{images/timeline_edit_insp_nav.pdf}
    \caption{Timeline}
    \label{fig:timeline}
\end{figure*}

==> tables/correlation_corsi_activity.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{l|lrr}
    
    \toprule
    \multicolumn{2}{l}{}&  Understanding & Navigation \\
    \midrule
         \multirow{3}{*}{\makecell{Corsi\\Score}}
         & 	Corr. Coefficient & -0.134&	0.195\\
         \cline{2-4}
	     & $p$&		0.437&	0.258\\
      \cline{2-4}
      & $N$& 19& 19\\
	     \bottomrule
    \end{tabular}
    \caption{Correlation of Corsi Block test score with time spent on Understanding and Navigation}
    \label{tab:correlation_corsi_activity}
\end{table*}

==> tables/correlation_corsi_perform.tex <==
\begin{table}[h]
    \centering
        \caption{Correlation of Corsi Block test score with time and file and annotation  accuracy}
    \label{tab:correlation}
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{l|lrrrr}
    \toprule
    \multicolumn{2}{l}{}&  $T$ & $A_{F}$ & $A_{AN}$\\
    \midrule
         \multirow{2}{*}{\makecell{Corsi\\Score}}
         & 	Correlation Coefficient & 0.141&	0.025&	0.025\\
         \cline{2-5}
	     & \textit{\textbf{p}}&		\textbf{0.415}&	\textbf{0.887}&	\textbf{0.887}\\
	     \bottomrule
    \end{tabular}

\end{table}

==> tables/correlation_feedback.tex <==
\begin{table*}[h]
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{l|lrr}
    \toprule
    \multicolumn{2}{l}{}&  Canvas Feedback (helpful?) & Canvas Order (0=unordered, 1=ordered)\\
    \midrule
         \multirow{2}{*}{\makecell{Corsi\\Score}}
         & 	Corr. Coefficient & -0.219&	-0.096\\
         \cline{2-4}
	     & $p$&		0.458&	0.745\\
	     \bottomrule
    \end{tabular}
    \caption{Correlation of Corsi Block test score with time and file and annotation  accuracy}
    \label{tab:correlation}
\end{table*}

